Reconstruction of the Higgs mass in events with Higgs bosons decaying into a pair of tau leptons using matrix element techniques

We present an algorithm for the reconstruction of the Higgs mass in events with Higgs bosons decaying into a pair of tau leptons. The algorithm is based on matrix element (ME) techniques and achieves a relative resolution on the Higgs boson mass of typically 15-20%. A previous version of the algorithm has been used in analyses of Higgs boson production performed by the CMS collaboration during LHC Run 1. The algorithm is described in detail and its performance on simulated events is assessed. The development of techniques to handle tau decays in the ME formalism represents an important result of this paper.

==> Makefile <==
HN  := hepnames
HPN := heppennames
HNN := hepnicenames

PDFLATEX := pdflatex --interaction=nonstopmode
LATEX := latex "\scrollmode\input"
DVIPS := dvips

ifndef V
OUTPUT := > /dev/null 2> /dev/null
#$(info OUTPUT = $(OUTPUT))
endif

.PHONY: all pdf ps clean

all: pdf $(HN).tar.gz
	@true

pdf: $(HN).pdf $(HNN)-rm.pdf $(HNN)-it.pdf $(HPN)-rm.pdf $(HPN)-it.pdf
	@true

ps: $(HN).ps $(HNN)-rm.ps $(HNN)-it.ps $(HPN)-rm.ps $(HPN)-it.ps
	@true

$(HN).tar.gz: README ChangeLog $(wildcard *.sty) $(wildcard *.pdf) $(wildcard *.tex) mkmacrotables Makefile
	@echo "Building $@ archive"
	tar czf $@ README ChangeLog *.sty *.pdf *.tex mkmacrotables Makefile

%.pdf: %.tex $(HNN)-macros.tex $(HPN)-macros.tex $(wildcard *.sty)
	@echo "Running pdflatex on $< ..."
	@$(PDFLATEX) $< $(OUTPUT)

%.ps: %.dvi
	@echo "Running dvips on $< ..."
	@$(DVIPS) $< $(OUTPUT)

%.dvi: %.tex $(HNN)-macros.tex $(HPN)-macros.tex $(wildcard *.sty)
	@echo "Running latex on $< ..."
	@$(LATEX) $< $(OUTPUT)

$(HNN)-macros.tex $(HNN)-rm.tex $(HNN)-it.tex $(HPN)-macros.tex $(HPN)-rm.tex $(HPN)-it.tex : $(wildcard *.sty) mkmacrotables
	@echo "Running mkmacrotables to generate code -> symbol tables"
	@./mkmacrotables

clean:
	rm -f *.tar.gz *.tgz *.dvi *.log *.aux *.pdf *.ps *.tmp *-macros.tex *-rm.tex *-it.tex

